Conversational Recommendation: Theoretical Model and Complexity Analysis

Recommender systems are software applications that help users find items of interest in situations of information overload in a personalized way, using knowledge about the needs and preferences of individual users. In conversational recommendation approaches, these needs and preferences are acquired by the system in an interactive, multi-turn dialog. A common approach in the literature to drive such dialogs is to incrementally ask users about their preferences regarding desired and undesired item features or regarding individual items. A central research goal in this context is efficiency, evaluated with respect to the number of required interactions until a satisfying item is found. This is usually accomplished by making inferences about the best next question to ask to the user. Today, research on dialog efficiency is almost entirely empirical, aiming to demonstrate, for example, that one strategy for selecting questions is better than another one in a given application. With this work, we complement empirical research with a theoretical, domain-independent model of conversational recommendation. This model, which is designed to cover a range of application scenarios, allows us to investigate the efficiency of conversational approaches in a formal way, in particular with respect to the computational complexity of devising optimal interaction strategies. Through such a theoretical analysis we show that finding an efficient conversational strategy is NP-hard, and in PSPACE in general, but for particular kinds of catalogs the upper bound lowers to POLYLOGSPACE. From a practical point of view, this result implies that catalog characteristics can strongly influence the efficiency of individual conversational strategies and should therefore be considered when designing new strategies. A preliminary empirical analysis on datasets derived from a real-world one aligns with our findings.

==> charts/hours.tex <==
\pgfplotsset{compat=1.16}
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{axis}[
    every axis plot post/.style={/pgf/number format/fixed},
    ybar=10pt,
    bar width=12pt,
    ymin=0,
    axis on top,
    ymax=10,
    xtick=data,
    axis y line=none, 
    axis x line=bottom,
    enlarge x limits=0.7,
    legend pos = north west,
    symbolic x coords={itemset1, itemset2},
    restrict y to domain*=0:12, % Cut values off at 220
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
        },
    nodes near coords={%
            \pgfmathprintnumber{\rawy}% Print unclipped values
        },
    axis lines*=left,
    clip=false
    ]
\addplot coordinates {(itemset1, 7.24) (itemset2, 72)}; 
\addplot coordinates {(itemset1, 7.40) (itemset2, 4.43)};
\legend{Protocol 1, Protocol 2}; 
\end{axis} 
\end{tikzpicture}
\caption{Execution Time (hours)\francesco
{for all users, and all preferred items, given one at a time as test item?}}
\label{plot:computation_time}
\end{figure}


==> charts/max.tex <==
\pgfplotsset{compat=1.16}
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{axis}[
    every axis plot post/.style={/pgf/number format/fixed},
    ybar=10pt,
    bar width=12pt,
    ymin=0,
    axis on top,
    ymax=500,
    xtick=data,
    axis y line=none, 
    axis x line=bottom,
    enlarge x limits=0.7,
    legend pos = north west,
    symbolic x coords={itemset1, itemset2},
    restrict y to domain*=0:550, % Cut values off at 220
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
        },
    nodes near coords={%
            \pgfmathprintnumber{\rawy}% Print unclipped values
        },
    axis lines*=left,
    clip=false
    ]
\addplot coordinates {(itemset1, 239.7415563) (itemset2, 3083.875993)}; 
\addplot coordinates {(itemset1, 205.9531457) (itemset2, 340.7572848)};
\legend{Protocol 1, Protocol 2}; 
\end{axis} 
\end{tikzpicture}
\caption{MAX Questions}
\label{plot:max_questions}
\end{figure}


==> sections/backup.tex <==
\vspace{10pt}
OLD TEXT
\vspace{3pt}
\hrule
\color{gray}

In this experiment the interaction is driven by the \crs.
For each user in the dataset we create the set of positively-rated items (PRI), consisting of items whose rating is greater than or equal to the user's average rating.  For each item $I$ in PRI, we simulate a dialog
%\dietmar{Terminology: What is an experiment? The entire thing? One configuration where we have one I as ``test item''?}
in which $I$ is the \emph{test item} (i.e., the only \emph{ideal} item.
%\dietmar{So this is the only ideal item in terms of the terminology from above? Terminology should be aligned.}
The dialog ends when the system recommends the selected test item (which the truthfully acting user will always accept). %\dietmar{We should repeat that we assume that the user will accept the item}
{\color{blue}Since we have to simulate an interaction between a system and a real user in a cold-start situation, we use the information related to the items $\hat{I}\in\text{PRI}\setminus\{I\}$ to simulate user's responses to system's questions. In case the system asks for the user's preference about a specific feature's value $\hat{v_i}$, we simulate that the user likes $\hat{v_i}$ if there is an item $\hat{I} \in \text{PRI}\setminus\{I\}$ such that $f_i(\hat{I}) = \hat{v_i}$. In case this latter condition does not hold we simulate the user dislikes $\hat{v_i}$.}




{\color{gray}In our evaluation protocols, we assume the user does not know in advance if the item she has in mind is available within the catalog or not. The interaction between the user and the systems, as well as the selection of the test item (i.e., the item we want to recommend), reflects this assumption.}


For each simulated dialog, all items in PRI except for $I$ are omitted from the catalog \C. In this way, we decouple \emph{efficiency} from efficacy: since the item that has to be found is always in \C, we concentrate only on the number of interactions (\ie questions) needed to find it.
%\tommaso{To be clarified and made more explicit.}
%\francesco{Where do we say that ``all items in PRI except for $I$ are omitted from the catalog \C. In this way, we decouple \emph{efficiency} from efficacy: since the item that has to be found is always in \C, we concentrate only on the number of interactions needed to find it.'' --- should we add this here? }
%\dietmar{I changed ``experiment configuration'' to ``(simulated) dialog'' above. What I don't understand is why we remove all items in PRI from the catalog. The single ideal item for a given is determined, why would having other possibly relevant items, which are not the target in the current run, be a problem? Maybe I am lost here.}

For each configuration there is a multi-turn dialog where the system asks a question on a feature (\eg ``What is your favorite director'') and the user answers by choosing a value from a set of \emph{active values} (AV).
%\dietmar{A dialog where the system asks a/one question? Shouldn't this be plural?}
The AV set changes during the interaction and is obtained through the intersection between all the possible values for the asked feature in the user's PRI %\dietmar{But we removed everything from PRI except I? }
and all the values in the set of recommendable items. As a result, the user cannot answer with a value that is not present in any recommendable object. After each user answer, a set of items is discarded from the set of recommendable items (\eg if the user answers ``Quentin Tarantino'' as favorite director, all the items with a different director are no longer recommendable and are discarded).
{\color{blue}The strategy we implemented for choosing the question to ask and the value to answer (from AV) is purely random. %\dietmar{This is not too convincing or logically following. Trying to confirm results does not imply that random values should be chosen.}
In this way, we avoid introducing other parameters\footnote{Notably, how to compute a DT, and since optimal DTs are hard to compute, how to approximate an optimal DT.} in our study. We recall that the worst case of a random DT is never worse than the worst DT; and on the other hand, the average case of a random DT is an average over all possible DTs.}

When the system has no more questions to ask (\ie, when all the features were asked), a recommendation is shown.
%\dietmar{We probably should discuss this in the meeting. According to the text above, the system asks for desired feature values, removes all items that do not have that value and the asks for the next feature value. At subsequent steps, only answers are possible that lead to a non-empty set of recommendations. So either the dialog ends and there is a movie that has all the desired features, or the user at some stage has no more feature value s/he can state to prefer. Which means we have to go back. So how can the next situation happen that a recommendation is rejected, as the user cannot specify a set of features that lead to an empty result set? }
The recommendation is rejected when the test item is missing from the list of recommendations.
If the recommendation is rejected, the recommended items are removed from the dataset, and the system runs a new round of questions.
%\dietmar{But we would not start from scratch, would we? Maybe this is all okay and corresponds to the Algorithm, but it should then be made clearer why this corresponds to P1. Above, P1 is characterized as a protocol where the system does not ask questions about disliked features after a rejection.}
Conversely, when the recommendation succeeds (the test item is in the list of recommendations), we choose another item, and we simulate a new dialog until all the items in PRI were selected once as test item.
This is  protocol P1.
%\dietmar{The above descriptions need revisions. Besides other aspects, I suggest to disentangle one individual experiment run (ie the search for one item) from the ``outer loop'', where each item is used as target/ideal item. I also found the last paragraph quite confusing. Also, it is only mentioned at the very end that this is P1. Why not repeating upfront, this is P1, it does <<repeat main idea>. Again, how is A1 related to P1?}

Regarding  protocol P2, the only difference compared to P1 is that when the recommendation is rejected, the user can declare she dislikes one of the feature values of the recommended item.
Such a ``dislike'' can happen for one of two reasons: (1) the user had not chosen a value for that feature because the CRS did not ask that; otherwise, (2) the user changes her mind on a liked value because it leads to unwanted items.

It is worth noting that the case in which the recommendation set is empty never occurs.
%\dietmar{Yes, but this very confusing here.}
In fact, when the CRS is not able to further distinguish a set of items (all the feature values are the same), it shows the whole set as recommendations. %\dietmar{The whole set means all items that fulfill the user preferences stated so far?}
%Such a ``dislike'' can happen for one of two reasons: (1) if it was not a value chosen by the user---because it was the only choice left, once the user had made the other choices---then it is really a value she dislikes; otherwise, (2) if it was a value the user declared to like, she now dislikes it because it leads to unwanted items. \dietmar{or no results?} \dietmar{The writing is confusing to me. We should lay out the goals that lead to the experiment designs in the beginning. This should naturally follow from the goals of the experiment, which are not very clearly stated above.}
When the user declares she dislikes a given feature value, all the other previous preferences are kept.  As an example, in the case the user answered ``Quentin Tarantino'' as favorite director, she can replace this value with another one (\eg ``Woody Allen'') chosen from the AV set. The values for the other features (e.g., genre, music composer, etc.) are kept. Such a protocol P2 always enters Line~\ref{alg:feature-value-reject} in Algorithm~\ref{algo-upper-bound}.

%Since the goal of our experimental evaluation is to provide evidence to \dietmar{Not sure we can confirm anything here. We can provide evidence that supports our theoretical claims} our theoretical results,

\color{black}
\vspace{3pt}
END OLD TEXT
\vspace{10pt}
\hrule


==> sections/problemDefinition.tex <==
\todo{DJ: Do we need that? Or covered in previous section?}
%Problem definition 

==> unusedParts/buildingDTs.tex <==
\begin{comment}

\renewcommand{\algorithmicrequire}{\textbf{Input:}} % in order to write "input" and "output" instead of "requires" and "ensure"
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[ht]
\caption{ComputeDT($\S,k$)}\label{algo-dt}
\begin{algorithmic}[1]
\Require a set of items \S, 
%a conversation state $U = \Vector{Q,\K,\P,\N}$, 
and an integer $k$
\Ensure \Vector{\T,k} where \T is a decision tree whose depth is at most $k$
\State Let $N$ be a new node
\If{(\S = \{I\})} \Comment{\S is a singleton}
\State Let $I$ be the label of $N$
\State \Return \Vector{N,1}
\Else
\State choose $f \in F$ such that $|AV(\S,f)|> 1$ \label{alg-dt:nondet}
\Comment{Nondeterministic choice}
\State Let $f$ be the label of $N$ 
\State Let $k = 0$
\For{each $v \in AV(\S,f)$} \label{alg-dt:for}
\State Let $\S'= \{I \in \S ~|~ f(I)=v \}$
\State Let $F' = \{ f \in F ~|~ |AV(\S',f)| > 1 \}$ \label{alg-dt:shorterF}
\State Let $\Vector{N',k'}= ComputeDT(\S',F')$
\State $k = \max(k,k')$
\State attach to $N$ an edge $(N,v,N')$
\EndFor
\State \Return \Vector{N,k}
\EndIf
\end{algorithmic}
\end{algorithm}
The time complexity of the above recursive algorithm 
\begin{theorem}
Given a catalog \C, with $p$ features $f_1,f_2,\ldots,f_p$, where the maximum cardinality of a feature domain is $K$, Algorithm~\ref{alg-dt:nondet} runs in nondeterministic polynomial time, using $O(p\cdot\log(K))$ space.
\end{theorem}
\begin{proof}
\francesco{I don't know if we can cite a textbook for the time complexity. A quick run on Google did not gave me the answer, so I repeat this standard proof here. The space complexity is what I need below, and this is less known.}
Each node corresponds to a recursive call. Every internal node of the tree has at least two children (Line~\ref{alg-dt:nondet}: the branching factor is $|AV(\S,f)|> 1$), so it is a branching node, and the number of leaves is $|\C|$. It is well known that the number of nodes (including leaves) in such a tree is $2|\C|-1$, which equals the number of recursive calls.

Regarding space, the total height of the recursive call stack cannot exceed $p$ since each recursive call leaves out from $F'$ (Line~\ref{alg-dt:shorterF}) at least the feature chosen in Line~\ref{alg-dt:nondet} (once a value $v$ for a feature $f$ is chosen, $v$ is the only active value for $f$). Moreover, in each recursive call, one needs a $\log(K)$-bits counter for enumerating feature values (Line~\ref{alg-dt:for}), hence the total space is $O(p\cdot \log(K)$.
\end{proof}
\end{comment}

==> unusedParts/strategies-old1.tex <==
%Devising optimal strategies
% subsection "strategies"
Our goal is to study conversation strategies for \crs.
For our setting, a \crs \emph{strategy} is an algorithm that, in every possible state of a conversation, suggests the system its next action, among the ones formalized above.
As discussed in Section~\ref{sec:rel_work}, the efficiency of a \crs strategy can be studied in terms of the number of interactions with the user needed to reach an item $I$, which we write in symbols as \inter. One can consider the worst case, \ie the maximum number of interactions (for some ``difficult'' item), or the average case, with respect to a probability distribution $\mathcal{P}:\C \rightarrow [0..1]$ estimating how likely item $I$ will be the chosen one. Such an average case gives rise to an \emph{expected} number of interactions, computed as $\Sigma_{I \in \C} \inter\cdot \mathcal{P}(I)$. In the rest of this paper, we will be agnostic about such a probability distribution, in the sense that our results hold for any distribution. However, when it is necessary to make an assumption, we assume the uniform distribution over items.

To study conversation strategies, we need some reasonable assumptions about how the user answers the system prompts. In our work, we assume that there is a  set $\I$ of \emph{ideal} items---unknown to the system and possibly partly unknown to the user too---which, if recommended by the \crs, would satisfy the user. 
Since we are studying efficiency, we assume that $\I \cap \C \neq \emptyset$, meaning that there always exist an item in the catalog that would satisfy the user, and the only point is how many interactions are needed to find it. Observe also that we do not set $\I \subset \C$, \ie we assume that there are ``ideal'' items the user would like, but which are not available in the catalog. They are exactly such items that make search difficult, since the user might drive the search (in the conversation) towards such unavailable items, heading towards available ones only later on.

%Observe that the realistic case is when $\frac{|\I \cap \C|}{|\C|} = \pi \ll 1$, \ie only very few items in \C would satisfy the user. In fact, consider the very simple strategy of proposing one item at random, and repeat until an item is chosen. From probability theory, the expected number of interactions for such a strategy is $\frac{|\C|+1}{|\I|+1} \approx \frac{1}{\pi}$.

%So from now on, we assume that $\pi \ll 1$, that is, the ideal items to be found in \C---if any---are very sparse in \C.

We assume that the user, during the conversation, adopts (even unintentionally) the following \emph{truthful attitude} when interacting with the \crs:
\begin{itemize}
    \item the user chooses a slot filling $\sigma(x) = v$ for a feature $f_i$,  \emph{if and only if} there is at least one ideal item $I \in \I$ whose feature $f_i$ is actually filled by $v$---in symbols, $\exists I\in \I : f_i(I) = v$. Note that this is a double implication, \ie if there is no such an ideal item, the user does not choose (or accepts as a suggestion)  to fill the slot $f_i$ with value $v$;

    \item similarly for slot change (revision): the user chooses (or accepts the suggestion) the change of a slot value $\tau(v) = w$ for a feature $f_i$,  \emph{if and only if} there is at least one ideal item $I \in \I$ such that  $f_i(I) = w$; 
    
    \item user's like/dislike statements about whole items are always coherent with ideal items \I, \ie when the user states that he/she likes an item $I$, it is $I \in \I$, and  when the user states that he/she dislikes an item $I$, then $I \not\in \I$. 
\end{itemize}

%We now introduce an important notion about user's choices. Intuitively, users can be more or less \emph{selective}: we now make this intuition more precise. We say that a user is \emph{most selective on \C} when there is no pair of items $I_1, I_2 \in \I \cap \C$ such that $I_1$ and $I_2$ share the same value for some feature $f$. Observe that this characteristic depends on the catalog \C; in the unrealistic case of a catalog containing an item for every possible combination of features, the only effective and efficient strategy for a most selective user would be to ask all $p$ features. However, in realistic cases, just a subset of features may select some item in \C (not the same features for every item, of course).


\subsection{Efficient Conversational Recommenders and Decision Trees}
\francesco{Maybe we can skip this title and go directly to "lower Bounds"}

\subsection{Lower Bounds} 

We first show that our problem of devising efficient strategies for \crs includes Binary Decision Trees (BDT) minimization as a special case.
A standard consequence of such an inclusion between problems is that every complete algorithm for devising an optimal strategy for \crs, could be used to minimize a BDT, hence, conversely, every lower bound on the complexity of BDT minimization (which is an NP-complete problem) is also a lower bound for computing optimal conversation strategies.

 
We recall the definition of a BDT \cite{Moret82} for our purposes. A BDTs is a procedural representation of a \emph{decision table}, whose definition we start with. A decision table is a tabular representation of a function whose domain is $B^p$ and whose range is the set of decisions. Given integers $p$, and $q \le 2^p$, a Decision Table is a $q \times p$ Boolean matrix\footnote{The use of the symbol $p$ (the same symbol used for the number of features in our formalization) is intentional here, as it will be clear later on.} in which the $p$ columns represent conditions/tests that can be \true or \false, and the $q$ rows represent the combinations of such conditions---one of which has to be assessed to take the appropriate decision. Each decision could be associated to one or more rows---all the combinations of conditions in which this decision has to be taken---and rows corresponding to impossible combinations are usually omitted. We give an example in Table~\ref{tab:example:DT:BDT}.
\begin{table}
\begin{tabular}{c|c}
    \begin{tabular}{cccc}
$x_1$   & $x_2$     & $x_3$ &  decision \\ \hline
\false  & \false    & \false    & $d_1$ \\
\false  & \false    & \true     & $d_1$ \\
\false  & \true     & \false    & $d_2$ \\
\false  & \true     & \true     & $d_3$ \\
\true   & \false    & \false    & $d_4$ \\
\true   & \true     & \false    & $d_4$ \\
\true   & \false     & \true    & $d_5$ \\
\true   & \true     & \true     & $d_5$
\end{tabular} 
     & 
\adjustbox{valign=m}{%
\begin{tikzpicture}
[
    level 1/.style={sibling distance=10em},
    level 2/.style={sibling distance=5em},
    level distance          = 4em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
  \node {$x_1$?}
    child  { node {$x_2$?}
        child { node {$d_1$}
        edge from parent node [left, above] {\false}
        }
        child { node {$x_3$?}
            child { node {$d_2$}
            edge from parent node [left, above] {\false}
            }
            child { node {$d_3$}
            edge from parent node [right, above] {\true}
            }
        edge from parent node [right, above] {\true}
        }
    edge from parent node [left, above] {\false}
    }
    child { node {$x_3$?}
        child { node {$d_4$}
        edge from parent node [left, above] {\false}
        }
        child { node {$d_5$}
        edge from parent node [right, above] {\true}
        }    
    edge from parent node [right, above] {\true} };
\end{tikzpicture}
}
\end{tabular}
\caption{A decision table (left) and a possible, optimized BDT representing it (right), whose expected cost is (2+3+3+2+2)/5=2.4}\label{tab:example:DT:BDT}
\end{table}

A BDT is a strategy for testing the conditions that leads to a decision in every situation.
In particular, the tree contains a test in each internal node, a label \true/\false in each arc, and a decision in every leaf (possibly repeated). The procedural interpretation of the BDT is: starting from the root, test the condition in the node, and proceed along the arc labeled with the result of the test. Repeat until a leaf is reached, which represents the decision to be taken. The \emph{cost} of the decision taken is the number of tests performed\footnote{In the general case each test may have its own different cost, and each combination of conditions may have a probability attached to it, but this is irrelevant here.}, which coincides with the length of the path from the root to that leaf. For a given table, there can be several BDT representing it, and BDT minimization is the problem of finding a BDT with a minimum cost. Usually, the cost is averaged over all leaves \cite{HyafilR76}, yielding a search for the minimum \emph{expected} cost. The decision problem related to such optimization problem is: Given a decision table and an integer $k$, is there a BDT representation of the table whose expected cost is $\le k$?


To show that  BDT minimization is a particular form of the problem of devising optimal \crs strategies, given a decision table $q \times p$ we fix a catalog of $q$ items, each with $p$ Boolean features. 
Decisions are one-one with items, so $|\C|$, \ie one-one with items conditions/tests  are one-one with  Boolean features. The \crs begins the conversation from a cold-start state in which no preference is known yet. More precisely,
\begin{itemize}
    \item the query  contains only variables: $Q_0 = \Vector{x_1,x_2,\ldots,x_p}$;
    \item the constraints $p$-vector $\K_0 = \Vector{\emptyset,\emptyset,\ldots,\emptyset}$ \ie it is a $p$-vector of empty sets;
    \item $\P_0 = \N_0 = \emptyset$, too.
\end{itemize}
Moreover, the answers given by the user always lead to an item that exists in the catalog, that is, $\I \subseteq \C$, so that once the system eventually proposes an item (after a conversation in which the user has the truthful attitude explained above), the user accepts it.
In this situation, the minimal interaction sequences that are possible are the ones in which only slot-filling is performed, going from the root of the tree to a chosen item in a leaf.
Such conversations composed solely by slot-fillings on Boolean features are equivalent to paths of a BDT. A lower bound on the efficiency of such conversations is also a lower bound for any conversational strategy.
Similarly to the literature on Decision Trees, we  concentrate on their \emph{average case}: is it possible to devise a strategy whose expected number of interactions (slot-fillings) is less than or equal to a given bound? 
Expected conversation length seems a better measure than maximum (worst-case) length, since we consider  strategies to be optimal also when few inefficient (\ie lengthy) conversations are outnumbered by many more efficient (\ie very short) ones.

Borrowing from results about the complexity of finding optimal BDTs, we can prove below that the problem of finding an efficient \crs strategy is  NP-hard in general, since it includes a problem which is NP-complete.

\begin{theorem}\label{thm-np-hardness}
The following problem is NP-hard: ``given an integer $k$, a specific user with its ideal items \I, a catalog \C, an initial state $U_0 + \Rec(U_0)$, where $U_0 = \Vector{Q_0,\K_0,\P_0,\N_0,}$, and $Q_0 = \Vector{x_1,x_2,\ldots,x_p}$, the constraints $\K_0$ are a $p$-vector of empty sets, and $\P_0 = \N_0 = \emptyset$,
is there a conversation strategy made only of slot-filling questions, such that the expected number of interactions with the user is less than or equal to $k$?''
\end{theorem}

\begin{proof}
We give a polynomial reduction from the following NP-complete problem \cite{HyafilR76}: given a set of objects $O_1,\ldots,O_c$, and a set of tests $T_1,\ldots,T_p$, such that each test returns \true for exactly three objects, decide whether there is a  BDT whose internal nodes are the tests, whose leaves are the objects, and whose external path length (\ie the sum of the lengths of all the paths from the root to a leaf) is less or equal to a given length $\ell$.

Given an instance of the source problem as above, we construct the target problem in Conversational Recommendation. Let the catalog $\C$ be made by $c$ items: for each object $O$, there is an item $I_O$. 
\dietmar{Unclear to me, is each $O \in C$? What is the (purpose of the) $I_O$ thing? Maybe the term test should also be explained above and more background given. Why exactly three objects? }\francesco{It is a bijection between problems, usually you do not use directly the objects of the source problem as elements of the target problem. 3 objects because this is the NP-hard problem: Exact-3-cover. If every feature selects only 2 items, the problem is not NP-hard anymore.}

We let the Boolean features be one-one with tests \dietmar{Not sure about clear understandability ``one-one'' phrase. }, \francesco{Again, it is a bijection, "tests" are not directly features in Recommenders, but for each test, you use a feature.}

\ie  $f_i = T_i$, for $i=1,\ldots,p$ while the items are defined as $I_O = \Vector{T_1(O),\ldots,T_p(O)}$
\ie each feature $f_i$ of an item $I_O$ has the same value as the one returned by Test $T_i$ on Object $O$.

We now prove that there exists a BDT solving an instance of the source problem, whose external path length is less than or equal to $\ell$---or equivalently, an expected path length of $\ell/c$---if and only if there is an efficient strategy for the target \crs, whose expected number of slot-filling interactions is less than or equal to $\ell/c$.
Without loss of generality, we represent the strategy of the \crs as a binary tree, too.

\textbf{Only-if-direction $\Longrightarrow$.} Suppose there exists such a BDT. Then define an efficient strategy as follows:
take the BDT $T$, and substitute test labels $T_i$ in the internal nodes with feature labels $f_i$ whose filling should be asked to the user, leaving edge connections untouched (\true/\false test results in BDT are one-one with \true/\false user filling in the \crs strategy). Then substitute each leaf node of the BDT, marked with object O, with a leaf marked by item $I_O$.

\textbf{If-direction $\Longleftarrow$.}
Suppose now that there exists an efficient \crs strategy for the target problem defined above---with $p$ Boolean features and $c$ items---whose expected number of questions is within $b$.

We prove that such a strategy defines a  BDT whose external path length is $\ell = b\cdot c$ as follows: transform the binary tree representing the strategy by substituting each internal-node feature label $f_i$ with test $T_i$, and each leaf-node item label $I_O$ with object $O$. Clearly such a BDT is isomorphic to the strategy, hence its expected path length is $b$, and so its external path length is $b \cdot c = \ell$.
\end{proof}

\dietmar{We could add an example of a slot-filling problem in the form a BDIT in a figure.}

The above theorem highlights the difficulty in optimizing \crs efficiency in the case in which the only transformation is slot-filling; one may wonder how representative of the general case such ``simple'' case is, and whether interactions with contractions/revisions could be more efficient than slot-filling, after all.
The following  theorem shows that the other transformations are just ``deroutes'' from the shortest interaction paths, showing that conversations containing contractions/revisions can always be transformed into conversations containing only slot-filling, whose length is no worse than the initial one.

\begin{theorem}\label{thm-only-slot-filling}
    For every sequence of interactions from $U_0 + \Rec(U_0)$ to a success state $U_n + \{I\}$, there is another sequence of interactions $U_0' + \Rec(U_0'), \ldots, U_m' + \{I\}$, whose transformations are only substitutions (slot fillings), and whose number of interactions is not larger than the initial one, \ie $m \le n$.
\end{theorem}
\begin{proof}
If the interaction is already composed by substitutions only, the claim is trivially true; suppose then that there are also contraction (slot-unfilling) and revision (slot-changing) interactions. For every contraction $\sigma(v) = x$, we focus on the state in which the feature contained $v$. If $f_i(Q_0) = v$, \ie the value was in the initial query $Q_0$, let $Q_0' = \tau(Q_0)$ where $\tau(v) = x$, that is, we start with the variable unfilled from the very beginning. If instead the filling happened in an intermediate interaction, we just remove the interaction in which $f_i$ was (erroneously) filled by $v$. Of course, we eliminate also the subsequent slot unfilling interaction. In both cases, the new sequence of interactions is shorter (by 1 or by 2) than $n$. We proceed in a similar way also for slot changing, and repeat the steps until no more such steps are performed. In the end, we obtain an interaction sequence that starts from $U_0' + \Rec(U_0')$ (with $U_0$ possibly different from $U_0$), ends with the same successful item at $U_m' + \{I\}$, where $m \le n$.
\end{proof}

The above theorem tells us that the shortest possible conversations include the ones in which only slot-filling is performed. Such conversations are the lucky ones, because there is no contraction/revision of the slot-fillings made. The goal of the \crs in this case is just to ask the least number of slot fillings leading to one item to propose, and stop. Hence, the above theorem evidences the significance of our NP-hardness reduction for \crs s in general. We now make some points about this result.

\subsubsection{Discussion of the NP-hardness result}
We stress that we are not interested in the above proof by itself, but in how it enriches the understanding of the computational problem of efficiency in \crs, thanks to the following observations:
\begin{enumerate}
    \item The problem is NP-hard for the case in which each \true feature selects three items. This means that NP-hardness does not depend on \emph{feature entropy}, that would be maximal when a feature selects half the catalog. Note also that since the original reduction \cite{HyafilR76} is from \textsc{exact-3-cover}, and the more general problem \textsc{exact-cover} is NP-hard too, our problem is NP-hard when a feature selects \emph{at least} three items.
    %This includes situations in which some features are hierarchically structured, \eg a feature about the director's nationality (``Do you like French directors?'') that is implied by a more specific feature (``Do you like Truffaut?''). The hard problem remains for features that are orthogonal, in the sense that they do not imply each other.
    % ??? notably, if each feature would select only two items, there would be polynomial-time algorithms for constructing optimal BDT.
    
    \item hardness is instead entangled with catalog \emph{incompleteness}, that is, the fact that not all combinations of feature values correspond to an available item; for (although irrealistic) complete catalogs, optimal decision trees can be constructed in time polynomial in the catalog size \cite{guij-etal-IPL99}.
    
    \item The proof does not mention how the tree is represented, only the decision whether there exists such a tree or not. Hence, NP-hardness holds also in the case in which the tree is represented implicitly, as a circuit (or a neural network) which, given a state of the conversation, suggests the next feature to fill. This is usually called a \emph{succinct} representation \cite{papa-yann-86} of a tree.
    %A different problem is to study how the size of the tree grows with the size of the problem (items, features). Such a problem has been proven non-approximable, as well as the problem of learning such trees \cite{hancock-IC-96}.

    \item Observe that there are at most ${{c}\choose{3}}$ possible different tests, hence $p \in O(n^3)$ in big-O notation---\ie the number of features is bounded by a (low) polynomial in $c$. This means that NP-hardness shows up even when the number of features $p$ and the number of items are polynomially related.
    
    \item The proof does not rely on the existence of more than one user; hence the problem is NP-hard even if we want to devise an efficient strategy only for one particular user (or, equivalently, for non-personalized \crs).
    
    \item The complexity analysis confirms the intuition  that cold start is a worst case for \crs. When some features in $Q$ contain a value, or \P and \N are not empty, this prunes some parts of the decision tree (of course, the problem remains NP-hard in the size of the remaining features and items). Many solutions have been proposed to alleviate such a cold-start problem, however, as markets expand  to new entries (in terms of both users and items), cold-start situations seem unavoidable, and algorithms that devise efficient strategies should cope with such situations.

    \item Theorems~\ref{thm-np-hardness} and~\ref{thm-only-slot-filling} together show that, although the conversation is composed by actions of slot-filling, slot-unfilling and revision, \emph{the problem of devising an efficient strategy is not a problem of optimal planning} of the order of such actions. However, slot-unfilling and revision are fundamental for another dimension of \crs evaluation, namely, \emph{effectiveness}: when slot-filling comes to a dead end, only the other two actions may steer  the conversation out of that dead end, and look for an acceptable alternative recommendation.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Upper Bounds}\label{sec:upper-bounds}

We now study the upper bound of the complexity of devising efficient strategies for \crs. We represent slot-filling strategies by (general) Decision Trees (DT), which are trees whose internal nodes can have more than two outgoing edges. Rephrasing the definition of binary decision trees of the previous section, our tree contains a feature $f$ in each internal node, a label with a value $v$ filling $f$ in each arc outgoing from the node, and an item in every leaf (possibly repeated). 
An example of a catalog and a possible slot-filling strategy for the conversation (represented as a DT) is given in Table~\ref{tab:example:DT}.



\begin{table}[htb]
\begin{tabular}{c|c}
    \begin{tabular}{llll}
director    & starring  & genre     & movie        \\ \hline
Spielberg   & Hanks     & historical & Forrest Gump \\
Spielberg   & Dreyfuss  & action    & Jaws         \\
Eastwood    & Hanks     & action    & Sully
\end{tabular} 
     & 
\adjustbox{valign=m}{%
\begin{tikzpicture}
[
    level 1/.style={sibling distance=10em},
    level 2/.style={sibling distance=5em},
    level distance          = 4em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
\node {director?}
    child { node {starring?}
        child { node {Forrest Gump}
        edge from parent node [left, above] {Hanks}
        }
        child { node {Jaws}
        edge from parent node [right, above] {Dreyfuss}
        }
    edge from parent node [left, above] {Spielberg}
    }
    child { node {Sully}
    edge from parent node [right, above] {Eastwood}
    }
;
\end{tikzpicture}
}
\end{tabular}
\caption{A catalog (left) and a possible, optimized, conversational strategy (right) represented as a DT. Note that two features are sufficient to distinguish all items.}\label{tab:example:DT}
\end{table}

The strategy represented by the DT is: starting from the root, ask the user to fill with a preferred value the feature in the node, and proceed along the arc labeled with the user's answer. Repeat until a leaf is reached, which identifies the item to propose. The \emph{expected cost} of such a (part of) conversation is the expected number of feature fillings asked to the user---\ie the average path length from the root to a leaf in the DT. 
We recall that the problem of finding an optimal strategy (in terms of expected number of interactions) for slot-filling is trivially NP-complete \cite{HyafilR76}: it is NP-hard, because it contains BDT optimization (see previous section) as a special case, and it belongs to NP because the DT representing the strategy is polynomial in the size of the catalog---hence a nondeterministc Turing Machine (TM) can compute such an optimal DT in polynomial time. Following the literature in complexity, we recall that an \emph{NP-oracle} is a black-box that, given as input an instance of an NP-complete problem, can compute in constant time a solution for it---usually called a \emph{guess} in Complexity Theory jargon. The class $\Delta^p_2$ (also called $P^{NP}$) is the class of problems solvable by a deterministic TM in polynomial time, that can use an NP-oracle during the computation\footnote{Note that since the TM works in polynomial time, also the number of times it can use the NP-oracle is limited by a polynomial.}. When the P-time TM can use the NP-oracle only a number of times that is limited by a \emph{logarithm} of the input, the corresponding class of problems is denoted by $\Theta^p_2$ (also called $\Delta^p_2[\log n]$). Clearly, $NP \subseteq \Theta^p_2 \subseteq \Delta^p_2$. We note that such complexity classes are not as abstract as they may seem, since natural problems for both classes have been found in the literature \cite{hema-etal-JACM97,papa-JACM84,Krentel88}. We make use of these notions in what follows.

Clearly if the user rejects the item, either slot unfilling or slot change must be performed. 
Intuitively, every slot unfilling (contraction) or slot change (revision) yields a ``restart'' of the slot-filling strategy, with a little more information: at least one item has been rejected by the user. It can therefore be added to the set \N the user dislikes, and will not be proposed again.
This incrementality in \N mirrors a reduction of the items to propose in \C, and leads to a trivial upper bound in the complexity of the problem of devising an optimal conversation strategy: Each item could be proposed at the end of a slot-filling series of interactions, and each new slot-filling (with a smaller catalog) can use  a  new strategy---represented by a DT---for choosing again the features to fill. The new strategy is motivated by the fact that once an item has been removed, the optimal strategy for the remaining items may change: for example in Table~\ref{tab:example:DT}, once the item ``Jaws'' has been removed, the new optimal trees have depth 1. 
After all possible items in the catalog have been proposed and rejected, the conversation must stop. Therefore, the problem can be solved by a deterministic TM that accesses an NP-oracle to guess an optimal DT when needed---that is, it belongs to $\Delta^p_2$. We prove this intuition in detail in the theorem below, and from the proof, we show that in a particular subclass of input catalogs, the upper bound on the complexity of the problem lowers to $\Theta^p_2$. 

\begin{theorem}\label{thm-upper-bound}
The following problem is in $\Delta_2^p$: ``Given a catalog \C of items, and an initial conversation state $U_0 + R(U_0)$, with $U_0 = \Vector{Q_0,\K_0,\P_0,\N_0}$, \emph{find} a strategy for the \crs which is optimal with respect to the expected number of interactions''.
%that concludes the conversation (either with a chosen item $I \in \C$, or with no item) within $M$ interactions on average?''
\end{theorem}
\begin{proof}
First of all, observe that a trivial strategy  is to propose each item in the catalog in turn; such a strategy needs  \emph{at most} $|\C|$ interactions (so less than $|\C|$ on average). Hence any optimal strategy cannot last more than $|\C|$ interactions on average. 
%hence, the problem makes sense only if $M < |\C|$, since otherwise the answer is trivially ``yes''. This fact is used at the end of the proof.

We prove the claim by \emph{(i)} exhibiting the strategy expressed by Algorithm~\ref{algo-upper-bound} below, that resorts on an NP-oracle, and \emph{(ii)} proving that it runs in polynomial time, given that the call of the NP-oracle uses constant time.
Recall that $\Rec(U)$ returns a list of recommended items coherent with $U$; in particular, $\Rec(U) \subseteq \C - \N$ (no item the user does not want is recommended), and for all $I \in \Rec(U): \forall i=1,\ldots,p : f_i(I) \not\in C_i  $ (if a user dislikes a particular feature value, no item with that feature value is proposed).

\dietmar{Line 5: How would we guess a decision tree, how would we know the expected interaction length? More information seems helpful.}\francesco{The guess is an abstraction of the process of solving an NP-complete problem. Since it is an abstraction, there is no "how". Regarding the interaction length, maybe you're right. let's delete all that part. So now Algorithm 1 is no more a decision algorithm, with yes/no answer; it is the strategy itself.}

\renewcommand{\algorithmicrequire}{\textbf{Input:}} % in order to write "input" and "output" instead of "requires" and "ensure"
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[ht]
\caption{Strategy for \crs}\label{algo-upper-bound}
\begin{algorithmic}[1]
\Require an initial conversation state $U_0 + R(U_0)$, with $U_0 = \Vector{Q_0,\K_0,\P_0,\N_0}$
%, and a maximum number of interactions $M$
%\Ensure ``yes'' if there is a strategy whose expected number of interactions is $\le M$, ``no'' otherwise
\State Let $j \gets 0$ be a counter
%\State\label{guess-k} \textbf{guess} an integer $k \le M$, and $k$ integers $h_1,h_2,\ldots,h_k \le M$ such that $h_1 + h_2 + \cdots + h_k = M$
\Repeat\label{alg:begin-iteration}
\State $j \gets j+1$
\State call the NP-oracle to get a Decision Tree $DT_j$ for the set of items $\C - \N_j$, 
\State\label{alg:use-DT} prompt the user to fill features in the order suggested by $DT_j$, leading to the proposal of one (or more) item $I \in R(U_j)$;
\If{the user rejects $I$}
    \State let $U_{j+1} = \Vector{Q_{j+1},\K_{j+1},\P_{j+1},\N_{j+1}}$ be as follows:
    \State $\P_{j+1} \gets \P_j$
    \State $\N_{j+1} \gets \N_j \cup \{I \}$
    \If{the user dislikes a particular feature value $v = f_i(I)$ of the rejected item $I$}\label{alg:feature-value-reject}
    \State let $C_i' \gets C_i \cup \{v\}$
    \State let $\K_{j+1} = \Vector{C_1,\ldots,C_i',\ldots,C_p}$
    \State $\N_{j+1} \gets \N_{j+1} \cup \{I' | v = f_i(I') \}$
        \If{$D_i - C_i' \neq \emptyset$}
        \State let $\tau(v) \doteq t$, where either $t \in (D_i-C_i)$ (slot change) or $t \in X$ (slot unfilling)
        \State let $Q_{j+1} \gets \tau(Q_j)$\\
                \Comment{no else: if the user rejected all possible values in $D_i$ execution will stop at Line~\ref{alg:end-iteration}}
        \EndIf
    \Else\label{alg:reject-as-a-whole}
    \State\label{alg:reject-as-a-whole-next} $Q_{j+1} \gets Q_j$, $\K_{j+1} \gets \K_j$
    \EndIf
\EndIf
\Until {(the user accepts the proposed item $I$) \textbf{or} ($\C-\N=\emptyset$) \textbf{or} ($C_i = D_i$ for some $i$)}\label{alg:end-iteration}
\end{algorithmic}
\end{algorithm}

It is easy to prove that Algorithm~\ref{algo-upper-bound} repeats its iterative part (Lines~\ref{alg:begin-iteration}--\ref{alg:end-iteration}) a number of times that is bounded by a polynomial in the input size. The worst case for this algorithm is that the user and the \crs explore the catalog, and find, eventually, that no item can satisfy the user's needs.
The claim immediately follows from the fact that in each iteration, at least one item $I$ is inserted in \N, and hence, eliminated from $\C-\N$. Clearly, the number of iterations is bounded by the number of items in the catalog \C, hence by a polynomial in $|\C|$.

Regarding the optimality of Algorithm~\ref{algo-upper-bound}, let  $E(Y)$ denote the expected value of a probabilistic variable $Y$. Observe that the number of interactions of Algorithm~\ref{algo-upper-bound} is a probabilistic variable $X = X_1 + X_2 + \cdots X_k$, where each $X_j$ is the probabilistic variable expressing the number of interactions in Line~\ref{alg:use-DT}, that is, the number of interactions of each optimal Decision Tree $DT_j$ , whose expected number of interactions is denoted by $E(X_j)$. Since  it is well known that $E(X) = E(X_1) + E(X_2) + \cdots + E(X_k)$, and each $E(X_j)$ is optimal for the items $\C-\N_j$ (items remaining at iteration $j$), $E(X)$ is optimal too.

We conclude that Algorithm~\ref{algo-upper-bound} is an optimal strategy for a \crs, using a polynomial number of calls to an NP oracle, each call depending on the results of the previous calls. Hence devising such an optimal strategy is a problem belonging to $\Delta_2^p$.
\end{proof}

The above lower and upper bounds restrict the complexity of finding efficient strategies for \crs between NP (lower bound) and $\Delta_2^p$ (upper bound). Although the two bounds do not match, the gap between them is considered the ``normal'' difference between decision and optimization for NP-complete problems \cite{Krentel88,GasarchKR95}. Since the aim of this paper is to bridge \crs practical efficiency with theoretical results, we leave investigation of this gap to future (more theoretically-oriented) research.
On the practical side, our $\Delta_2^p$ upper bound ensures that usual techniques for solving NP-complete problems, and in particular, finding optimal DT---\eg Mixed-Integer Optimization \cite{bert-dunn-ML17}, branch-and-bound search \cite{agli-etal-AAAI2020}, SAT and MAXSAT encoding \cite{naro-etal-IJCAI18}---can be used for devising optimal conversational strategies, while our NP lower bound ensures that employing such techniques is not an overshoot.


It is interesting to note that when the user rejects a particular feature value---\eg ``I don't like green phones'', as taken into account in Line~\ref{alg:feature-value-reject}---this fact rules out more than one item (all the items with the same feature value), thus improving the worst case of the conversation. We prove in what follows that such a difference in the interaction carries over to a difference in the complexity class the efficiency problem belongs to, backing up intuition, but highlighting when such intuition fails. For this part, we recall $\theta$-notation: for a function $f(n)$, we write  $f(n) \in \theta(g(n))$ if both $f(n) \in O(g(n))$, and $f(n) \in \Omega(g(n))$, \ie $f(n)$ grows no faster than $g(n)$, but also there are infinitely many (worst) cases in which $f(n)$ grows as fast as $g(n)$.

\begin{corollary}
Let the problem and the initial conditions be the ones of Theorem~\ref{thm-upper-bound}. Moreover, let the cardinality of all domains be bounded by a constant $k = max_i(|D_i|)$, and suppose $|\C| \in \theta(k^p)$. If, whenever the user rejects a proposed item, s/he also points to a particular feature value of that item s/he dislikes, then the problem belongs to $\Theta_2^p$.
\end{corollary}
\begin{proof}
Membership in $\Theta_2^p$ is proved using the same Algorithm~\ref{algo-upper-bound} above, plus the fact that in every iteration of the algorithm, the condition in Line~\ref{alg:feature-value-reject} is satisfied, hence neither the check of the ``if'' condition is needed, nor Lines~\ref{alg:reject-as-a-whole}--\ref{alg:reject-as-a-whole-next}.

Clearly, the cardinality of the input catalog \C is bounded by $k^p$ (there cannot be more items than all possible $p$ combinations of feature values). After $k-1$ iterations, each ruling out a value for a feature, the number of remaining items is bounded by $k^{p-1}$ (all the possible values for a feature have been eliminated, but one). When the values ruled out belong to different features, the expression is more complex than $k^{p-1}$, but in any case, after at most $p\cdot (k-1)$ iterations, all values but one have been ruled out for each feature. At that point, either the user accepts the item whose feature values are the last remaining in each domain, or the user rejects it, and in any case the conversation concludes.

Let $n$ denote the size of the input catalog (we neglect the size of the initial state, since it is dominated by the former one). Since $n \in \theta(k^p)$, $\log(n) \in \theta(p\cdot\log(k)) = \theta(p)$ if $k$ is a constant. Hence, the number of iterations $p(k-1) \in \theta(p) = \theta(\log(n)) \subset O(\log(n))$.
\end{proof}

The above result backs up \crs  implementations whose strategies enforce the following interaction: whenever the user rejects a proposed item, the \crs asks the user whether there is a particular feature value of that item s/he dislikes, and discards all items with the same feature value.

However, observe that the above result holds only in the situation in which the input catalog has a number of items that is comparable with $k^p$---\ie items are ``dense'' in the space of features---and increases because more features $f_{p+1}, f_{p+2},\ldots$ are added---\ie more domains $D_{p+1}, D_{p+2}, \ldots$ are added---not because each domain $D_i$ of each feature value increases its cardinality. If, instead of considering $k$ as a constant, we would consider $p $ as a constant, the drop in complexity due to the strategy of always asking for a disliked feature value, would not show up\footnote{Modifying the line of reasoning at the end of the proof, one could show that the number of interactions is polynomial in this case.}. In other words, when the number $p$ of features is fixed, and the catalog increases because more possible values are added to each feature, asking to rule out such values one by one is not exponentially more efficient than asking to rule out items one by one. Hence, our theoretical analysis points out which characteristics of the catalog must be evaluated when implementing efficient  strategies for a \crs: if the catalog is composed by items with few features, and lots of possible values in each feature, the strategy of asking always to rule out a value when rejecting an item does not yield an exponential increase in efficiency; if instead the catalog is made by items described by lots of features, each feature with few values, such a strategy could improve efficiency in a complexity-theoretical provable way.
\dietmar{Maybe we should highlight this last part a bit more.}\francesco{The next section is intended to highlight this in a practical case. What more? Any suggestion is welcome.}
In the next section, we show such a difference in a practical setting.


==> unusedParts/strategies-old2.tex <==
%Devising optimal strategies
% subsection "strategies"
Our goal is to study conversation strategies for \crs.
For our setting, a \crs \emph{strategy} is an algorithm that, in every possible state of a conversation, suggests the system its next action, among the ones formalized above.
As discussed in Section~\ref{sec:rel_work}, the efficiency of a \crs strategy can be studied in terms of the number of interactions with the user needed to reach an item $I$, which we write in symbols as \inter. One can consider the worst case, \ie the maximum number of interactions (for some ``difficult'' item), or the average case, with respect to a probability distribution $\mathcal{P}:\C \rightarrow [0..1]$ estimating how likely item $I$ will be the chosen one. Such an average case gives rise to an \emph{expected} number of interactions, computed as $\Sigma_{I \in \C} \inter\cdot \mathcal{P}(I)$. In the rest of this paper, we will be agnostic about such a probability distribution, in the sense that our results hold for any distribution. However, when it is necessary to make an assumption, we assume the uniform distribution over items.

To study conversation strategies, we need some reasonable assumptions about how the user answers the system prompts. In our work, we assume that there is a  set $\I$ of \emph{ideal} items---unknown to the system and possibly partly unknown to the user too---which, if recommended by the \crs, would satisfy the user. 
Since we are studying efficiency, we assume that $\I \cap \C \neq \emptyset$, meaning that there always exist an item in the catalog that would satisfy the user, and the only point is how many interactions are needed to find it. Observe also that we do not set $\I \subset \C$, \ie we assume that there are ``ideal'' items the user would like, but which are not available in the catalog. They are exactly such items that make search difficult, since the user might drive the search (in the conversation) towards such unavailable items, heading towards available ones only later on.

%Observe that the realistic case is when $\frac{|\I \cap \C|}{|\C|} = \pi \ll 1$, \ie only very few items in \C would satisfy the user. In fact, consider the very simple strategy of proposing one item at random, and repeat until an item is chosen. From probability theory, the expected number of interactions for such a strategy is $\frac{|\C|+1}{|\I|+1} \approx \frac{1}{\pi}$.

%So from now on, we assume that $\pi \ll 1$, that is, the ideal items to be found in \C---if any---are very sparse in \C.

We assume that the user, during the conversation, adopts (even unintentionally) the following \emph{truthful attitude} when interacting with the \crs:
\begin{itemize}
    \item the user chooses a slot filling $\sigma(x) = v$ for a feature $f_i$,  \emph{if and only if} there is at least one ideal item $I \in \I$ whose feature $f_i$ is actually filled by $v$---in symbols, $\exists I\in \I : f_i(I) = v$. Note that this is a double implication, \ie if there is no such an ideal item, the user does not choose (or accepts as a suggestion)  to fill the slot $f_i$ with value $v$;

    \item similarly for slot change (revision): the user chooses (or accepts the suggestion) the change of a slot value $\tau(v) = w$ for a feature $f_i$,  \emph{if and only if} there is at least one ideal item $I \in \I$ such that  $f_i(I) = w$; 
    
    \item user's like/dislike statements about whole items are always coherent with ideal items \I, \ie when the user states that he/she likes an item $I$, it is $I \in \I$, and  when the user states that he/she dislikes an item $I$, then $I \not\in \I$. 
\end{itemize}

%We now introduce an important notion about user's choices. Intuitively, users can be more or less \emph{selective}: we now make this intuition more precise. We say that a user is \emph{most selective on \C} when there is no pair of items $I_1, I_2 \in \I \cap \C$ such that $I_1$ and $I_2$ share the same value for some feature $f$. Observe that this characteristic depends on the catalog \C; in the unrealistic case of a catalog containing an item for every possible combination of features, the only effective and efficient strategy for a most selective user would be to ask all $p$ features. However, in realistic cases, just a subset of features may select some item in \C (not the same features for every item, of course).


\subsection{Efficient Conversational Recommenders and Decision Trees}
\francesco{Maybe we can skip this title and go directly to "lower Bounds"}

\subsection{Lower Bounds} 

We first show that our problem of devising efficient strategies for \crs includes Binary Decision Trees (BDT) minimization as a special case.
A standard consequence of such an inclusion between problems is that every complete algorithm for devising an optimal strategy for \crs, could be used to minimize a BDT, hence, conversely, every lower bound on the complexity of BDT minimization (which is an NP-complete problem) is also a lower bound for computing optimal conversation strategies.

 
We recall the definition of a BDT \cite{Moret82} for our purposes. A BDTs is a procedural representation of a \emph{decision table}, whose definition we start with. A decision table is a tabular representation of a function whose domain is $B^p$ and whose range is the set of decisions. Given integers $p$, and $q \le 2^p$, a Decision Table is a $q \times p$ Boolean matrix\footnote{The use of the symbol $p$ (the same symbol used for the number of features in our formalization) is intentional here, as it will be clear later on.} in which the $p$ columns represent conditions/tests that can be \true or \false, and the $q$ rows represent the combinations of such conditions---one of which has to be assessed to take the appropriate decision. Each decision could be associated to one or more rows---all the combinations of conditions in which this decision has to be taken---and rows corresponding to impossible combinations are usually omitted. We give an example in Table~\ref{tab:example:DT:BDT}.
\begin{table}
\begin{tabular}{c|c}
    \begin{tabular}{cccc}
$x_1$   & $x_2$     & $x_3$ &  decision \\ \hline
\false  & \false    & \false    & $d_1$ \\
\false  & \false    & \true     & $d_1$ \\
\false  & \true     & \false    & $d_2$ \\
\false  & \true     & \true     & $d_3$ \\
\true   & \false    & \false    & $d_4$ \\
\true   & \true     & \false    & $d_4$ \\
\true   & \false     & \true    & $d_5$ \\
\true   & \true     & \true     & $d_5$
\end{tabular} 
     & 
\adjustbox{valign=m}{%
\begin{tikzpicture}
[
    level 1/.style={sibling distance=10em},
    level 2/.style={sibling distance=5em},
    level distance          = 4em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
  \node {$x_1$?}
    child  { node {$x_2$?}
        child { node {$d_1$}
        edge from parent node [left, above] {\false}
        }
        child { node {$x_3$?}
            child { node {$d_2$}
            edge from parent node [left, above] {\false}
            }
            child { node {$d_3$}
            edge from parent node [right, above] {\true}
            }
        edge from parent node [right, above] {\true}
        }
    edge from parent node [left, above] {\false}
    }
    child { node {$x_3$?}
        child { node {$d_4$}
        edge from parent node [left, above] {\false}
        }
        child { node {$d_5$}
        edge from parent node [right, above] {\true}
        }    
    edge from parent node [right, above] {\true} };
\end{tikzpicture}
}
\end{tabular}
\caption{A decision table (left) and a possible, optimized BDT representing it (right), whose expected cost is (2+3+3+2+2)/5=2.4}\label{tab:example:DT:BDT}
\end{table}

A BDT is a strategy for testing the conditions that leads to a decision in every situation.
In particular, the tree contains a test in each internal node, a label \true/\false in each arc, and a decision in every leaf (possibly repeated). The procedural interpretation of the BDT is: starting from the root, test the condition in the node, and proceed along the arc labeled with the result of the test. Repeat until a leaf is reached, which represents the decision to be taken. The \emph{cost} of the decision taken is the number of tests performed\footnote{In the general case each test may have its own different cost, and each combination of conditions may have a probability attached to it, but this is irrelevant here.}, which coincides with the length of the path from the root to that leaf. For a given table, there can be several BDT representing it, and BDT minimization is the problem of finding a BDT with a minimum cost. Usually, the cost is averaged over all leaves \cite{HyafilR76}, yielding a search for the minimum \emph{expected} cost. The decision problem related to such optimization problem is: Given a decision table and an integer $k$, is there a BDT representation of the table whose expected cost is $\le k$?


To show that  BDT minimization is a particular form of the problem of devising optimal \crs strategies, given a decision table $q \times p$ we fix a catalog of $q$ items, each with $p$ Boolean features. 
Decisions are one-one with items, so $|\C|$, \ie one-one with items conditions/tests  are one-one with  Boolean features. The \crs begins the conversation from a \emph{cold-start state} in which no preference is known yet. More precisely,
\begin{itemize}
    \item the query  contains only variables: $Q_0 = \Vector{x_1,x_2,\ldots,x_p}$;
    \item the constraints $p$-vector $\K_0 = \Vector{\emptyset,\emptyset,\ldots,\emptyset}$ \ie it is a $p$-vector of empty sets;
    \item $\P_0 = \N_0 = \emptyset$, too.
\end{itemize}
Moreover, the answers given by the user always lead to an item that exists in the catalog, that is, $\I \subseteq \C$, so that once the system eventually proposes an item (after a conversation in which the user has the truthful attitude explained above), the user accepts it.
In this situation, the minimal interaction sequences that are possible are the ones in which only slot-filling is performed, going from the root of the tree to a chosen item in a leaf.
Such conversations composed solely by slot-fillings on Boolean features are equivalent to paths of a BDT. A lower bound on the efficiency of such conversations is also a lower bound for any conversational strategy.
Similarly to the literature on Decision Trees, we  concentrate on their \emph{average case}: is it possible to devise a strategy whose expected number of interactions (slot-fillings) is less than or equal to a given bound? 
Expected conversation length seems a better measure than maximum (worst-case) length, since we consider  strategies to be optimal also when few inefficient (\ie lengthy) conversations are outnumbered by many more efficient (\ie very brief) ones.

Borrowing from results about the complexity of finding optimal BDTs, we can prove below that the problem of finding an efficient \crs strategy is  NP-hard in general, since it includes a problem which is NP-complete.

\begin{theorem}\label{thm-np-hardness}
The following problem is NP-hard: ``given an integer $k$, a specific user with its ideal items \I, a catalog \C, an initial cold-start state $U_0 + \Rec(U_0)$, where $U_0 = \Vector{Q_0,\K_0,\P_0,\N_0,}$, and $Q_0 = \Vector{x_1,x_2,\ldots,x_p}$, the constraints $\K_0$ are a $p$-vector of empty sets, and $\P_0 = \N_0 = \emptyset$,
is there a conversation strategy made only of slot-filling questions, such that the expected number of interactions with the user is less than or equal to $k$?''
\end{theorem}

\begin{proof}
We give a polynomial reduction from the following NP-complete problem \cite{HyafilR76}: given a set of objects $O_1,\ldots,O_c$, and a set of tests $T_1,\ldots,T_p$, such that each test returns \true for exactly three objects, decide whether there is a  BDT whose internal nodes are the tests, whose leaves are the objects, and whose external path length (\ie the sum of the lengths of all the paths from the root to a leaf) is less or equal to a given length $\ell$.

Given an instance of the source problem as above, we construct the target problem in Conversational Recommendation. Let the catalog $\C$ be made by $c$ items: for each object $O$, there is an item $I_O$. 
\dietmar{Unclear to me, is each $O \in C$? What is the (purpose of the) $I_O$ thing? Maybe the term test should also be explained above and more background given. Why exactly three objects? }\francesco{It is a bijection between problems, usually you do not use directly the objects of the source problem as elements of the target problem. 3 objects because this is the NP-hard problem: Exact-3-cover. If every feature selects only 2 items, the problem is not NP-hard anymore.}

We let the Boolean features be one-one with tests \dietmar{Not sure about clear understandability ``one-one'' phrase. }, \francesco{Again, it is a bijection, "tests" are not directly features in Recommenders, but for each test, you use a feature.}

\ie  $f_i = T_i$, for $i=1,\ldots,p$ while the items are defined as $I_O = \Vector{T_1(O),\ldots,T_p(O)}$
\ie each feature $f_i$ of an item $I_O$ has the same value as the one returned by Test $T_i$ on Object $O$.

We now prove that there exists a BDT solving an instance of the source problem, whose external path length is less than or equal to $\ell$---or equivalently, an expected path length of $\ell/c$---if and only if there is an efficient strategy for the target \crs, whose expected number of slot-filling interactions is less than or equal to $\ell/c$.
Without loss of generality, we represent the strategy of the \crs as a binary tree, too.

\textbf{Only-if-direction $\Longrightarrow$.} Suppose there exists such a BDT. Then define an efficient strategy as follows:
take the BDT $T$, and substitute test labels $T_i$ in the internal nodes with feature labels $f_i$ whose filling should be asked to the user, leaving edge connections untouched (\true/\false test results in BDT are one-one with \true/\false user filling in the \crs strategy). Then substitute each leaf node of the BDT, marked with object O, with a leaf marked by item $I_O$.

\textbf{If-direction $\Longleftarrow$.}
Suppose now that there exists an efficient \crs strategy for the target problem defined above---with $p$ Boolean features and $c$ items---whose expected number of questions is within $b$.

We prove that such a strategy defines a  BDT whose external path length is $\ell = b\cdot c$ as follows: transform the binary tree representing the strategy by substituting each internal-node feature label $f_i$ with test $T_i$, and each leaf-node item label $I_O$ with object $O$. Clearly such a BDT is isomorphic to the strategy, hence its expected path length is $b$, and so its external path length is $b \cdot c = \ell$.
\end{proof}

\dietmar{We could add an example of a slot-filling problem in the form a BDIT in a figure.}
\francesco{Binary features are somewhat unrealistic, I keep such an example (with non binary features) for the next section}
The above theorem highlights the difficulty in optimizing \crs efficiency in the case in which the only transformation is slot-filling; one may wonder how representative of the general case such ``simple'' case is, and whether interactions with contractions/revisions could be more efficient than slot-filling, after all.
The following  theorem shows that the other transformations are just ``deroutes'' from the shortest interaction paths, showing that conversations containing contractions/revisions can always be transformed into conversations containing only slot-filling, whose length is no worse than the initial one.

\begin{theorem}\label{thm-only-slot-filling}
    For every sequence of interactions from $U_0 + \Rec(U_0)$ to a success state $U_n + \{I\}$, there is another sequence of interactions $U_0' + \Rec(U_0'), \ldots, U_m' + \{I\}$, whose transformations are only substitutions (slot fillings), and whose number of interactions is not larger than the initial one, \ie $m \le n$.
\end{theorem}
\begin{proof}
If the interaction is already composed by substitutions only, the claim is trivially true; suppose then that there are also contraction (slot-unfilling) and revision (slot-changing) interactions. For every contraction $\sigma(v) = x$, we focus on the state in which the feature contained $v$. If $f_i(Q_0) = v$, \ie the value was in the initial query $Q_0$, let $Q_0' = \tau(Q_0)$ where $\tau(v) = x$, that is, we start with the variable unfilled from the very beginning. If instead the filling happened in an intermediate interaction, we just remove the interaction in which $f_i$ was (erroneously) filled by $v$. Of course, we eliminate also the subsequent slot unfilling interaction. In both cases, the new sequence of interactions is shorter (by 1 or by 2) than $n$. We proceed in a similar way also for slot changing, and repeat the steps until no more such steps are performed. In the end, we obtain an interaction sequence that starts from $U_0' + \Rec(U_0')$ (with $U_0$ possibly different from $U_0$), ends with the same successful item at $U_m' + \{I\}$, where $m \le n$.
\end{proof}

The above theorem tells us that the shortest possible conversations include the ones in which only slot-filling is performed. Such conversations are the lucky ones, because there is no contraction/revision of the slot-fillings made. The goal of the \crs in this case is just to ask the least number of slot fillings leading to one item to propose, and stop. Hence, the above theorem evidences the significance of our NP-hardness reduction for \crs s in general. We now make some points about this result.

\subsubsection{Discussion of the NP-hardness result}
We stress that we are not interested in the above proof by itself, but in how it enriches the understanding of the computational problem of efficiency in \crs, thanks to the following observations:
\begin{enumerate}
    \item The problem is NP-hard for the case in which each \true feature selects three items. This means that NP-hardness does not depend on \emph{feature entropy}, that would be maximal when a feature selects half the catalog. Note also that since the original reduction \cite{HyafilR76} is from \textsc{exact-3-cover}, and the more general problem \textsc{exact-cover} is NP-hard too, our problem is NP-hard when a feature selects \emph{at least} three items.
    %This includes situations in which some features are hierarchically structured, \eg a feature about the director's nationality (``Do you like French directors?'') that is implied by a more specific feature (``Do you like Truffaut?''). The hard problem remains for features that are orthogonal, in the sense that they do not imply each other.
    % ??? notably, if each feature would select only two items, there would be polynomial-time algorithms for constructing optimal BDT.
    
    \item hardness is instead entangled with catalog \emph{incompleteness}, that is, the fact that not all combinations of feature values correspond to an available item; for (although irrealistic) complete catalogs, optimal decision trees can be constructed in time polynomial in the catalog size \cite{guij-etal-IPL99}.
    
    \item The proof does not mention how the tree is represented, only the decision whether there exists such a tree or not. Hence, NP-hardness holds also in the case in which the tree is represented implicitly, as a circuit (or a neural network) which, given a state of the conversation, suggests the next feature to fill. This is usually called a \emph{succinct} representation \cite{papa-yann-86} of a tree.
    %A different problem is to study how the size of the tree grows with the size of the problem (items, features). Such a problem has been proven non-approximable, as well as the problem of learning such trees \cite{hancock-IC-96}.

    \item Observe that there are at most ${{c}\choose{3}}$ possible different tests, hence $p \in O(n^3)$ in big-O notation---\ie the number of features is bounded by a (low) polynomial in $c$. This means that NP-hardness shows up even when the number of features $p$ and the number of items are polynomially related.
    
    \item The proof does not rely on the existence of more than one user; hence the problem is NP-hard even if we want to devise an efficient strategy only for one particular user (or, equivalently, for non-personalized \crs).
    
    \item The complexity analysis confirms the intuition  that cold start is a worst case for \crs. When some features in $Q$ contain a value, or \P and \N are not empty, this prunes some parts of the decision tree (of course, the problem remains NP-hard in the size of the remaining features and items). Many solutions have been proposed to alleviate such a cold-start problem, however, as markets expand  to new entries (in terms of both users and items), cold-start situations seem unavoidable, and algorithms that devise efficient strategies should cope with such situations.

    \item Theorems~\ref{thm-np-hardness} and~\ref{thm-only-slot-filling} together show that, although the conversation is composed by actions of slot-filling, slot-unfilling and revision, \emph{the problem of devising an efficient strategy is not a problem of optimal planning} of the order of such actions. However, slot-unfilling and revision are fundamental for another dimension of \crs evaluation, namely, \emph{effectiveness}: when slot-filling comes to a dead end, only the other two actions may steer  the conversation out of that dead end, and look for an acceptable alternative recommendation.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Upper Bounds}\label{sec:upper-bounds}

We now study the upper bound of the complexity of devising efficient strategies for \crs. We represent slot-filling strategies by (general) Decision Trees (DT), which are trees whose internal nodes can have more than two outgoing edges. Rephrasing the definition of binary decision trees of the previous section, a decision tree for driving the conversation in a \crs contains a feature $f$ in each internal node, a label with a value $v$ filling $f$ in each arc outgoing from the node, and an item in every leaf (possibly repeated). 
An example of a catalog and a possible slot-filling strategy for the conversation (represented as a DT) is given in Table~\ref{tab:example:DT}.

\begin{table}[htb]
\begin{tabular}{c|c}
    \begin{tabular}{llll}
director    & starring  & genre     & movie        \\ \hline
Spielberg   & Hanks     & historical & Forrest Gump \\
Spielberg   & Dreyfuss  & action    & Jaws         \\
Eastwood    & Hanks     & action    & Sully
\end{tabular} 
     & 
\adjustbox{valign=m}{%
\begin{tikzpicture}
[
    level 1/.style={sibling distance=10em},
    level 2/.style={sibling distance=5em},
    level distance          = 4em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
\node {director?}
    child { node {starring?}
        child { node {Forrest Gump}
        edge from parent node [left, above] {Hanks}
        }
        child { node {Jaws}
        edge from parent node [right, above] {Dreyfuss}
        }
    edge from parent node [left, above] {Spielberg}
    }
    child { node {Sully}
    edge from parent node [right, above] {Eastwood}
    }
;
\end{tikzpicture}
}
\end{tabular}
\caption{A catalog (left) and a possible, optimized, conversational strategy (right) represented as a DT. Note that two features are sufficient to distinguish all items.}\label{tab:example:DT}
\end{table}

The strategy represented by the DT is: starting from the root, ask the user to fill with a preferred value the feature in the node, and proceed along the arc labeled with the user's answer. Repeat until a leaf is reached, which identifies the item to propose. The \emph{expected cost} of such a (part of) conversation is the expected number of feature fillings asked to the user---\ie the average path length from the root to a leaf in the DT. 
We recall that the problem of finding an optimal decision tree (in terms of expected number of interactions) is trivially NP-complete \cite{HyafilR76}: it is NP-hard, because it contains BDT optimization (see previous section) as a special case, and it belongs to NP because the DT representing the strategy is polynomial in the size of the catalog---hence a nondeterministc Turing Machine (TM) can compute such an optimal DT in polynomial time. 
We delve into the details of such a nondeterministc algorithm since they are needed later in this section.

First of all, observe that at any given point of the conversation, the focus is restricted to a set of items $\S \subseteq \C$ compatible with the answers of the user so far; for example, if a user tells the system that one of her most favourite directors is \textit{Spielberg}, the system concentrates on Spielberg's movies (the set \S) excluding (for the moment) the others. In such a set of items, each feature $f_i$ is not filled by all possible values in its domain $D_i$; continuing the example, the feature $f_{\mathit{Starring}}$ is filled by \textit{Hanks, Duvall}, but it is never filled by \textit{De Sica}, because there are no movies starring \textit{De Sica} whose director is Spielberg. We call such values \emph{Active Values} for $f_i$ in \S, written as $AV(\S,f_i)$. More formally, 
$AV(\S,f_i) = \{ v \in D_i ~|~ \exists I \in \S : v = f_i(I) \}$.
We make use of Active Values in the following algorithm, that will be used as a subprocedure later on.

\renewcommand{\algorithmicrequire}{\textbf{Input:}} % in order to write "input" and "output" instead of "requires" and "ensure"
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[ht]
\caption{ComputeDT($\S,k$)}\label{algo-dt}
\begin{algorithmic}[1]
\Require a set of items \S, 
%a conversation state $U = \Vector{Q,\K,\P,\N}$, 
and an integer $k$
\Ensure \Vector{\T,k} where \T is a decision tree whose depth is at most $k$
\State Let $N$ be a new node
\If{(\S = \{I\})} \Comment{\S is a singleton}
\State Let $I$ be the label of $N$
\State \Return \Vector{N,1}
\Else
\State choose $f \in F$ such that $|AV(\S,f)|> 1$ \label{alg-dt:nondet}
\Comment{Nondeterministic choice}
\State Let $f$ be the label of $N$ 
\State Let $k = 0$
\For{each $v \in AV(\S,f)$} \label{alg-dt:for}
\State Let $\S'= \{I \in \S ~|~ f(I)=v \}$
\State Let $F' = \{ f \in F ~|~ |AV(\S',f)| > 1 \}$ \label{alg-dt:shorterF}
\State Let $\Vector{N',k'}= ComputeDT(\S',F')$
\State $k = \max(k,k')$
\State attach to $N$ an edge $(N,v,N')$
\EndFor
\State \Return \Vector{N,k}
\EndIf
\end{algorithmic}
\end{algorithm}
The time complexity of the above recursive algorithm 
\begin{theorem}
Given a catalog \C, with $p$ features $f_1,f_2,\ldots,f_p$, where the maximum cardinality of a feature domain is $K$, Algorithm~\ref{alg-dt:nondet} runs in nondeterministic polynomial time, using $O(p\cdot\log(K))$ space.
\end{theorem}
\begin{proof}
\francesco{I don't know if we can cite a textbook for the time complexity. A quick run on Google did not gave me the answer, so I repeat this standard proof here. The space complexity is what I need below, and this is less known.}
Each node corresponds to a recursive call. Every internal node of the tree has at least two children (Line~\ref{alg-dt:nondet}: the branching factor is $|AV(\S,f)|> 1$), so it is a branching node, and the number of leaves is $|\C|$. It is well known that the number of nodes (including leaves) in such a tree is $2|\C|-1$, which equals the number of recursive calls.

Regarding space, the total height of the recursive call stack cannot exceed $p$ since each recursive call leaves out from $F'$ (Line~\ref{alg-dt:shorterF}) at least the feature chosen in Line~\ref{alg-dt:nondet} (once a value $v$ for a feature $f$ is chosen, $v$ is the only active value for $f$). Moreover, in each recursive call, one needs a $\log(K)$-bits counter for enumerating feature values (Line~\ref{alg-dt:for}), hence the total space is $O(p\cdot \log(K)$.
\end{proof}

Algorithm~\ref{algo-dt} could be used in \crs for a strategy using only slot-filling.
However, a single DT would be an incomplete strategy for \crs, since it does not consider the possibility of reject, and consequently, slot-unfilling and slot change. 
%Clearly if the user rejects the item, either slot unfilling or slot change must be performed. 
Intuitively, every slot unfilling (contraction) or slot change (revision) yield some sort of  ``restart'' of the slot-filling strategy, with a little more information: at least one item has been rejected by the user. It can therefore be added to the set \N the user dislikes, and will not be proposed again.
This incrementality in \N mirrors a reduction of the items to propose in \C, and leads to a trivial upper bound in the complexity of the problem of devising an optimal conversation strategy: each item could be proposed at most once. Observe that after a reject, the system might use a  new strategy---represented by a newer DT---for continuing the conversation. Such a  new strategy is motivated by the fact that once an item has been removed, the optimal strategy for the remaining items may change: for example in Table~\ref{tab:example:DT}, once the item ``Jaws'' has been removed, every new optimal tree has obviously depth 1. 
After all possible items in the catalog have been proposed and rejected, the conversation must stop. Therefore, deciding whether there is a strategy for a catalog \C that ends in at most $M$ interactions is a problem can be solved in PSPACE. We prove this intuition in detail in the theorem below, and from the proof, we show that in a particular subclass of input catalogs, the upper bound on the complexity of the problem lowers to PTIME. 

In order to study the upper bound of the complexity of devising strategies for \crs, we recall from Complexity Theory the following notions. An \emph{Alternating Turing Machine} (ATM) \cite{chan-etal-JACM81} is a TM in which states are partitioned into two categories: existential states, and universal states. An existential state accepts if at least one of its possible outgoing transitions leads to an accepting state; a universal state accepts if all its transitions lead to an accepting state. Existential states with no transition always reject, while universal states with no transition always accept. A non-deterministic TM is a special ATM in which all states with outgoing transitions are existential, and the only universal states are those with no transitions (accepting states).
The class of problems solved by an ATM whose time is bounded by $f(n)$ is called $ATIME(f(n))$ (alternating time); a well-known result relating ATMs and deterministic TMs is that $ATIME(f(n))=DSPACE(f(n))$, where $DSPACE(f(n))$ is the class of problems solvable by a (deterministic) TM using space bounded by $f(n)$. A consequence of this equivalence---that we are going to use below---is that if a problem can be solved by an ATM working in polynomial time, then the same problem can be solved by a TM in polynomial space, that is, the problem belongs to PSPACE.

ATMs have been used to prove several complexity results about strategies of 2-player games \cite{solt-wils-TCS11,bodl-JFCS91}, because existential states correspond to a player (``I have a move such that\ldots''), while universal states correspond to her opponent (``for every move of the opponent\ldots'')\footnote{In Chandra \& Stockmeyer's words \cite{chan-stoc-FOCS76}, ``Alternation corresponds to game-playing, much like nondeterminism corresponds to searching''.}. We make use too of this correspondence, in which the \crs choices are the existential states (``there is a feature to fill such that\ldots'') while the user's answers correspond to universal states (``for every possible user's answer\ldots'').

%We make use of these notions in what follows.


\begin{theorem}\label{thm-upper-bound}
The following problem is in PSPACE: ``Given a catalog \C of items, an integer $M$, and an initial conversation state $U_0 + R(U_0)$, with $U_0 = \Vector{Q_0,\K_0,\P_0,\N_0}$, \emph{is there} a strategy for the \crs which ends in at most $M$ interactions?''.
\end{theorem}
\begin{proof}
First of all, observe that a trivial strategy  is to propose each item in the catalog in turn; such a strategy needs  \emph{at most} $|\C|$ interactions. Hence the problem makes sense only if $M < |\C|$, since otherwise the answer is trivially ``yes''. 
%This fact is used at the end of the proof.

We prove the claim by \emph{(i)} exhibiting an ATM that returns \true if and only if such a strategy exists, where such an ATM is expressed at an abstract level by Algorithm~\ref{algo-upper-bound} below, and \emph{(ii)} proving that it runs in polynomial time.
%Recall that $\Rec(U)$ returns a list of recommended items coherent with $U$; in particular, no item the user does not want is recommended (in formulas, $\Rec(U) \subseteq \C - \N$), and if a user dislikes a particular feature value, no item with that feature value is proposed (formally, for all $I \in \Rec(U): \forall i=1,\ldots,p : f_i(I) \not\in C_i  $).

\begin{algorithm}[ht]
\caption{Strategy($\C,U, 
M$)}\label{algo-upper-bound}
\begin{algorithmic}[1]
\Require a catalog \C (fixed), a conversation state $U = \Vector{Q,\K,\P,\N}$, and an integer $M$
\Ensure
\begin{tabular}{|ll}
   \true  & if there is a strategy whose number of interactions is $\le M$ \\
   \false  & otherwise
\end{tabular} 
\If{$M \le 0$}
\Return \false \Comment{Base case 1: There is no strategy with 0 interactions}
\Else 
    \If{$|\C - \N| \le M$}
        \State \Return \true \Comment{Base case 2: Propose one by one items in $\C-\N$ (trivial strategy)}
    \Else
        \State Let \Vector{\T,m} = ComputeDT($\C-\N,m)$
        \For every item $I \in \C-\N$, whose depth in \T is $d \le m$
        \State Let $U' = \Vector{Q,\K,\P,\N\cup\{I\}}$
        \State Strategy($\C,U', M-m$) 
        \EndFor
    \EndIf
\EndIf
\end{algorithmic}
\end{algorithm}

It is easy to prove that Algorithm~\ref{algo-upper-bound} uses polynomial space, since in each recursive call, at least one item $I$ is inserted in \N, and hence, eliminated from $\C-\N$. Clearly, the height of the recursion stack is bounded by the number of items in the catalog \C, hence the total space is bounded by a polynomial in $|\C|$.


Regarding the optimality of Algorithm~\ref{algo-upper-bound}, let  $E(Y)$ denote the expected value of a probabilistic variable $Y$. Observe that the number of interactions of Algorithm~\ref{algo-upper-bound} is a probabilistic variable $X = X_1 + X_2 + \cdots X_k$, where each $X_j$ is the probabilistic variable expressing the number of interactions in Line~\ref{alg:use-DT}, that is, the number of interactions of each optimal Decision Tree $DT_j$ , whose expected number of interactions is denoted by $E(X_j)$. Since  it is well known that $E(X) = E(X_1) + E(X_2) + \cdots + E(X_k)$, and each $E(X_j)$ is optimal for the items $\C-\N_j$ (items remaining at iteration $j$), $E(X)$ is optimal too.

We conclude that Algorithm~\ref{algo-upper-bound} is an optimal strategy for a \crs, using a polynomial number of calls to an NP oracle, each call depending on the results of the previous calls. Hence devising such an optimal strategy is a problem belonging to $\Delta_2^p$.
\end{proof}

The above lower and upper bounds restrict the complexity of finding efficient strategies for \crs between NP (lower bound) and $\Delta_2^p$ (upper bound). Although the two bounds do not match, the gap between them is considered the ``normal'' difference between decision and optimization for NP-complete problems \cite{Krentel88,GasarchKR95}. Since the aim of this paper is to bridge \crs practical efficiency with theoretical results, we leave investigation of this gap to future (more theoretically-oriented) research.
On the practical side, our $\Delta_2^p$ upper bound ensures that usual techniques for solving NP-complete problems, and in particular, finding optimal DT---\eg Mixed-Integer Optimization \cite{bert-dunn-ML17}, branch-and-bound search \cite{agli-etal-AAAI2020}, SAT and MAXSAT encoding \cite{naro-etal-IJCAI18}---can be used for devising optimal conversational strategies, while our NP lower bound ensures that employing such techniques is not an overshoot.


It is interesting to note that when the user rejects a particular feature value---\eg ``I don't like green phones'', as taken into account in Line~\ref{alg:feature-value-reject}---this fact rules out more than one item (all the items with the same feature value), thus improving the worst case of the conversation. We prove in what follows that such a difference in the interaction carries over to a difference in the complexity class the efficiency problem belongs to, backing up intuition, but highlighting when such intuition fails. For this part, we recall $\theta$-notation: for a function $f(n)$, we write  $f(n) \in \theta(g(n))$ if both $f(n) \in O(g(n))$, and $f(n) \in \Omega(g(n))$, \ie $f(n)$ grows no faster than $g(n)$, but also there are infinitely many (worst) cases in which $f(n)$ grows as fast as $g(n)$.

\begin{corollary}
Let the problem and the initial conditions be the ones of Theorem~\ref{thm-upper-bound}. Moreover, let the cardinality of all domains be bounded by a constant $k = max_i(|D_i|)$, and suppose $|\C| \in \theta(k^p)$. If, whenever the user rejects a proposed item, s/he also points to a particular feature value of that item s/he dislikes, then the problem belongs to $\Theta_2^p$.
\end{corollary}
\begin{proof}
Membership in $\Theta_2^p$ is proved using the same Algorithm~\ref{algo-upper-bound} above, plus the fact that in every iteration of the algorithm, the condition in Line~\ref{alg:feature-value-reject} is satisfied, hence neither the check of the ``if'' condition is needed, nor Lines~\ref{alg:reject-as-a-whole}--\ref{alg:reject-as-a-whole-next}.

Clearly, the cardinality of the input catalog \C is bounded by $k^p$ (there cannot be more items than all possible $p$ combinations of feature values). After $k-1$ iterations, each ruling out a value for a feature, the number of remaining items is bounded by $k^{p-1}$ (all the possible values for a feature have been eliminated, but one). When the values ruled out belong to different features, the expression is more complex than $k^{p-1}$, but in any case, after at most $p\cdot (k-1)$ iterations, all values but one have been ruled out for each feature. At that point, either the user accepts the item whose feature values are the last remaining in each domain, or the user rejects it, and in any case the conversation concludes.

Let $n$ denote the size of the input catalog (we neglect the size of the initial state, since it is dominated by the former one). Since $n \in \theta(k^p)$, $\log(n) \in \theta(p\cdot\log(k)) = \theta(p)$ if $k$ is a constant. Hence, the number of iterations $p(k-1) \in \theta(p) = \theta(\log(n)) \subset O(\log(n))$.
\end{proof}

The above result backs up \crs  implementations whose strategies enforce the following interaction: whenever the user rejects a proposed item, the \crs asks the user whether there is a particular feature value of that item s/he dislikes, and discards all items with the same feature value.

However, observe that the above result holds only in the situation in which the input catalog has a number of items that is comparable with $k^p$---\ie items are ``dense'' in the space of features---and increases because more features $f_{p+1}, f_{p+2},\ldots$ are added---\ie more domains $D_{p+1}, D_{p+2}, \ldots$ are added---not because each domain $D_i$ of each feature value increases its cardinality. If, instead of considering $k$ as a constant, we would consider $p $ as a constant, the drop in complexity due to the strategy of always asking for a disliked feature value, would not show up\footnote{Modifying the line of reasoning at the end of the proof, one could show that the number of interactions is polynomial in this case.}. In other words, when the number $p$ of features is fixed, and the catalog increases because more possible values are added to each feature, asking to rule out such values one by one is not exponentially more efficient than asking to rule out items one by one. Hence, our theoretical analysis points out which characteristics of the catalog must be evaluated when implementing efficient  strategies for a \crs: if the catalog is composed by items with few features, and lots of possible values in each feature, the strategy of asking always to rule out a value when rejecting an item does not yield an exponential increase in efficiency; if instead the catalog is made by items described by lots of features, each feature with few values, such a strategy could improve efficiency in a complexity-theoretical provable way.
\dietmar{Maybe we should highlight this last part a bit more.}\francesco{The next section is intended to highlight this in a practical case. What more? Any suggestion is welcome.}
In the next section, we show such a difference in a practical setting.

